EMU/GAMA: Refining Dust Extinction Corrections for H{\alpha} Luminosity Functions Using Radio-Based Calibration

We present a novel approach to correcting H$\alpha$ luminosity functions for dust extinction by calibrating against radio-based star formation rates (SFRs), using data from the Evolutionary Map of the Universe (EMU) and Galaxy and Mass Assembly (GAMA) surveys. Accurate dust correction is essential for deriving SFRs from rest-frame UV-optical emission lines, particularly as the \textit{James Webb Space Telescope} extends such measurements to galaxies at $z>5$. While a luminosity dependence of dust obscuration has long been recognised, our method exploits the empirical relationship between obscured (H$\alpha$) and unobscured (radio) SFRs to provide a dust correction that can be applied where traditional spectroscopic techniques, e.g. Balmer line based approaches, are unavailable. We apply the SFR based dust correction to 25 published H$\alpha$ luminosity functions spanning $0<z<8$, and derive corresponding star formation rate densities (SFRDs). Adopting the locally calibrated H$\alpha$--radio relation ends up with an overestimate of the cosmic SFRD by more than two orders of magnitude at $z\gtrsim1$. Motivated by the luminosity dependent relation in the local Universe, we introduce a new model where the luminosity dependence of the dust obscuration decreases with increasing redshift. This approach can reproduce observed SFRDs across cosmic time. These results highlight the potential of a radio-based calibration for dust correction, where a luminosity dependent correction would need to decline in strength with increasing redshift. This implies that the dust content or distribution in galaxies at early epochs differs substantially from that in the local Universe.

==> Authors_Cambridge.tex <==
\author{\sn{Willingham} \gn{J.}$^{1,2}$, \sn{Hopkins} \gn{A.}$^{1,2}$, \sn{Zafar} \gn{T.}$^{1,2,3}$, \sn{Afonso} \gn{J.}$^{4,5}$, \sn{Ahmed} \gn{U.T.}$^{6,2,7}$, \sn{Ahmad} \gn{A.}$^{8}$, \sn{Battisti} \gn{A.}$^{9,10,3}$, \sn{Bomans} \gn{D.}$^{11,12}$, \sn{Brown} \gn{M. J. I.}$^{13}$, \sn{Cowley} \gn{M.}$^{14,15}$, \sn{Farrah} \gn{D.}$^{16,17}$, \sn{Galvin} \gn{T.J.}$^{18,19}$, \sn{Holwerda} \gn{B.}$^{20}$, \sn{Leahy} \gn{D.}$^{21}$, \sn{Maio} \gn{U.}$^{22,23}$, \sn{Mukherjee} \gn{T.}$^{1,2,3}$, \sn{Prathap} \gn{J.}$^{1,2,3}$, \sn{Seymour} \gn{N.}$^{24}$, \sn{Loon} \gn{J.Th. van}$^{25}$, \sn{Ward} \gn{E.}$^{1,2}$}

\affil{$^1$ School of Mathematical and Physical Sciences, 12 Wally's Walk, Macquarie University, NSW 2109, Australia \\ $^2$ Macquarie University Astrophysics and Space Technologies Research Centre, Sydney, NSW 2109, Australia \\ $^3$ ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO-3D), Australia \\ $^4$ Instituto de Astrofísica e Ciências do Espaço, Universidade de Lisboa, OAL, Tapada da Ajuda, 1349-018 Lisbon, Portugal \\ $^5$ Departamento de Física, Faculdade de Ciências, Universidade de Lisboa, Edifício C8, Campo Grande, 1749-016 Lisbon, Portugal \\ $^6$ Australian Astronomical Optics, Macquarie University, 105 Delhi Rd, North Ryde, NSW 2113, Australia \\ $^7$ Centre for Astrophysics, University of Southern Queensland, 37 Sinnathamby Boulevard, Springfield Central, QLD 4300, Australia \\ $^8$ School of Science, Western Sydney University, Locked Bag 1797, Penrith, NSW 2751, Australia \\ $^9$ Research School of Astronomy and Astrophysics, Australian National University, Weston Creek, ACT, Australia \\ $^10$ International Centre for Radio Astronomy Research (ICRAR), University of Western Australia, M468, Crawley, WA, Australia \\ $^11$ Ruhr Astroparticle and Plasma Physics Center (RAPP Center), 44780 Bochum, Germany \\ $^12$ Ruhr-Universität Bochum, Fakultät für Physik und Astronomie, Astronomisches Institut (AIRUB), 44780 Bochum, Germany \\ $^13$ School of Physics \& Astronomy, Monash University, Clayton, VIC, Australia \\ $^14$ School of Chemistry \& Physics, Faculty of Science, Queensland University of Technology, Brisbane, QLD 4000, Australia \\ $^15$ University of Southern Queensland, Centre for Astrophysics, West Street, Toowoomba QLD 4350, Australia \\ $^16$ Department of Physics and Astronomy, University of Hawai'i at Mānoa, 2505 Correa Road, Honolulu, HI 96822, USA \\ $^17$ Institute for Astronomy, University of Hawai'i, 2680 Woodlawn Dr., Honolulu, HI 96822, USA \\ $^18$ International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia \\ $^19$ CSIRO Space \& Astronomy, P.O. Box 1130, Bentley, WA 6102, Australia \\ $^20$ Leiden Observatory, Leiden University, NL-2300 RA Leiden, Netherlands \\ $^21$ Department of Physics and Astronomy, University of Calgary, Calgary, AB, Canada \\ $^22$ INAF – Osservatorio Astronomico di Trieste, Via Tiepolo 11, I-34143, Trieste, Italy \\ $^23$ IFPU – Institute for Fundamental Physics of the Universe, Via Beirut 2, I-34014, Trieste, Italy \\ $^24$ International Centre for Radio Astronomy Research, Curtin University, GPO Box U1987, Bentley, WA 6845, Australia \\ $^25$ Lennard-Jones Laboratories, Keele University, ST5 5BG, UK}
